A general framework for ensemble distribution distillation

Ensembles of neural networks have been shown to give better performance than single networks, both in terms of predictions and uncertainty estimation. Additionally, ensembles allow the uncertainty to be decomposed into aleatoric (data) and epistemic (model) components, giving a more complete picture of the predictive uncertainty. Ensemble distillation is the process of compressing an ensemble into a single model, often resulting in a leaner model that still outperforms the individual ensemble members. Unfortunately, standard distillation erases the natural uncertainty decomposition of the ensemble. We present a general framework for distilling both regression and classification ensembles in a way that preserves the decomposition. We demonstrate the desired behaviour of our framework and show that its predictive performance is on par with standard distillation.

==> Paper/Discussion/alt_loss.tex <==
\paragraph{Loss function alternatives}
Minimising the \nll in equation \eqref{eq:general_distillation_loss} has the potential to allow for fine-grained control over the distilled networks performance on
the two tasks of making predictions and representing uncertainty.
Despite that, it has no natural way of including the annotated data that does exist.

The predictive distribution in \eqref{eq:predictive_dist} can be used to design a loss term which takes the labelled data into account
\begin{align}
    \loss^{\text{pred}}(\varphi) = - \lambda \E_{p(x, y)} \log \tilde{q}( y; g_{\varphi}(x))
\end{align}

with $\lambda$ a tuning parameter. Then the trade-off between the accuracy of the distilled model and its ability to model uncertainty can be controlled by adding this  term to the total loss. This trade-off between the two tasks of the distilled model can also be used without the requirement of labelled data and instead with the aim to give the mean predictions a higher importance during training.

\paragraph{Training with out-of-distribution data} The defined framework does allow for training of the distilled model using data for which labels are not available. Hence, the performance of the distilled model on out-of-distribution data can be addressed by expansion of the training data set to include data points that are not in-distribution. In practice however, it can be difficult to construct a relevant OOD dataset for the training and we have not considered this option here.


==> Paper/Discussion/logit_matching_vs_temp_anneal.tex <==
\paragraph{Logits matching vs temperature annealing for classification}\label{sec:disc:temperature}
In the classification setting we have primarily considered parameterising $q(y;z)$ by parametrising $z$ as logits rather than probability vectors. 
Using a non-standard parametrisation can seem contrived, but it has potential advantages:

If we instead work with the standard parameterisation of $q$ in terms of the probability vector, then the distillation process can have difficulties in distinguishing small (but potentially important) differences in the class probabilities. This is due to the fact that the \softMax function squashes the unbounded logits into the interval $(0, 1)$, which can cause predictions to be close on the probability simplex even though they might be well separated in logit space. In \cite{standard_distill} they address this issue using \textit{temperature annealing} by temporarily increasing the temperature of the \softMax function during training. Performing the distillation directly in logit space provides another remedy to the same issue, and avoids the need to specify a temperature or annealing schedule. The importance of this flexibility is of interest for further study.

%The problem that distillation methods can have a hard time in capturing small differences in class probabilities has been recognised before. \cite{standard_distill} propose to use \textit{temperature annealing} to address this issue.
%The idea is to rescale the logits before applying the \softMax function, of both the distilled model and the target ensemble,
%\begin{equation}
 %   q_k = \frac{e^{z_k / %T}}{\sum_{k'} e^{z_{k'} / T}},
%    \label{eq:temp_softmax}
%\end{equation}
%where $T \geq 0$ is referred to as the temperature of the \softMax. 

%This tweak of the original distribution is expressly used in order to more easily distinguish differences in logit space,
%both for ordinary distillation \cite{standard_distill} and for distribution distillation \cite{prior_distr_distill}. 


==> Paper/Experiments/Classification/evaluating_distillation.tex <==
\subsection{Evaluation of distilled model - CIFAR10}
We provide an analysis of the distilled model's ability to fit to the ensemble logits in the classification setting.

\subsubsection{Comparing logit distributions}
We investigate how well the distilled model manages to mimic the ensemble by comparing its parameter predictions to the sample mean and variance over the ensemble logits on CIFAR-10 test data. In \cref{fig:class:param_eval} we display histograms of the average of the mean and variance over classes $1,...,K-1$
given a data point $x$, where the histogram is computed over all data points in the test set.

\begin{figure}
    \centering
    \input{Paper/Experiments/Classification/fig/logit_params.tikz}
     \caption{Histograms of the mean (\textit{left}) and variance (\textit{right}) given CIFAR-10 in-distribution test data as predicted by our distilled model and over the logits of the ensemble used to train it. The mean and variance are displayed as the average over the classes for each data point.}
         \label{fig:class:param_eval}
\end{figure}

The histograms can give us an idea of how well the distilled model represents the ensemble. From what can be observed in \cref{fig:class:param_eval},
the histograms over the mean values match very well, indicating that the distilled model manages to capture the mean of the ensemble logits.
The variance, which represents the epistemic uncertainty, also has a reasonable fit, although the variances predicted by the distilled model
seem to be somewhat overestimated.

\subsubsection{Comparing uncertainty estimates} A decomposition of uncertainty based on the predictions of the distilled model is performed in order to analyse the model's ability to capture aleatoric and epistemic uncertainty. For this, we use an entropy measure, and base our calculations on the general uncertainty measures in \cref{eq:dist:total_uncert}-\cref{eq:dist:aleatoric_uncert} and \cref{eq:epistemic_uncert}, using 100 samples from the distribution over $z$. In \cref{fig:class:entropy_eval}, we compare the uncertainty estimates to measures obtained from the ensemble. % in  histograms.

\begin{figure}
    \centering
    \input{Paper/Experiments/Classification/fig/entropy_decomposition.tikz}
     \caption{Histograms of aleatoric (\textit{left}) and epistemic (\textit{right})  uncertainty obtained on CIFAR-10 test data with our distilled model and the ensemble used to train it.}
         \label{fig:class:entropy_eval}
\end{figure}

Equivalently to the variance in logit space, \cref{fig:class:param_eval}, the distilled model has a tendency to overestimate the uncertainties. It would not be surprising if the higher entropy of the distilled model in output space is a direct reflection of the overestimation of the variance over $z_1, ..,, z_{K-1}$. 

%Naturally, there are several possible explanations to why the distilled model has not fully captured the true spread of the ensemble.
%In the experiments, we select a similar network architecture for the distilled model as the individual ensemble members.
%However, it might be the case that predicting both the mean and spread of the ensemble is a more complex task than the original one of predicting class probabilities.
%Hence, the objective at hand could require a more complex network architecture.
%Moreover the flexibility of the distilled model is affected by the distribution family of $v(z\vert x)$. Considering that the given framework does not limit us to the specific design choices made in these experiments, another distribution family might be more suitable for describing the ensemble. 

%Also relevant for the performance of the distilled model is the size of the ensemble.
%An ensemble size of 10 gives only a mere 10 samples from the distribution over the logits given a data point $x$.
%It could be hypothesised that the sample size is too small to allow for the distilled model to correctly estimate the covariance matrix of a multivariate normal distribution. In addition, the representation might not be good enough to generalise to the full in-distribution data. With this in mind, it would be of interest to investigate the effects of an increasing ensemble size on the models ability to capture the spread of the ensemble. \cite{prior_distr_distill} notes that an increasing ensemble size have quickly diminishing returns for a Dirichlet distribution but it is not clear if this is a general property.

==> Paper/Experiments/Classification/fig/full_acc_ece.tex <==
\includegraphics[]{Paper/Experiments/Classification/fig/acc_ece_test.eps}

\vspace{0.5em}$\!$\includegraphics[]{Paper/Experiments/Classification/fig/acc_benchmark_experiments_resnet20.eps}

\vspace{0.5em}\includegraphics[]{Paper/Experiments/Classification/fig/ece_benchmark_experiments_resnet20.eps}


==> mlsp_style_info.tex <==
% Authors


Single address.
---------------
\name{Author(s) Name(s)\thanks{Thanks to XYZ agency for funding.}}
\address{Author Affiliation(s)}
% 
For example:
------------
\address{%
    School \\
    Department \\
    Address
}

Two addresses.
--------------
\twoauthors{%
    A. Author-one, B. Author-two\sthanks{Thanks to XYZ agency for funding.}
}{%
    School A-B \\
    Department A-B \\
    Address A-B \\
    Email A-B
}{%
  C. Author-three, D. Author-four\sthanks{The fourth author performed the work while at ...}
}{%
    School C-D \\
    Department C-D \\
    Address C-D \\
    Email C-D
}

Two or more addresses (alternative form).
-----------------------------------------
If you need to list more than 2 authors or the option for two options above 
produces a poor author block, please use the following structure:
\name{%
    Author Name$^{\star \dagger}$%
    \qquad Author Name$^{\star}$%
    \qquad Author Name$^{\dagger}$\thanks{Thanks to XYZ agency for funding.}%
}
\address{%
    $^{\star}$ Affiliation Number One \\%
    $^{\dagger}$ Affiliation Number Two%
}

\section{Introduction}
\label{sec:intro}

These guidelines include complete descriptions of the fonts, spacing, and
related information for producing your proceedings manuscripts. Please follow
them.

Select one of the four copyright notices below and put in the text field below the first column (only required for the camera-ready paper submission). \textbf{Please pay attention to that most authors should use Copyright notice 4.}

\noindent{\bf Copyright notice 1:}\\
For papers in which all authors are employed by the US government, the copyright notice is:\\
{U.S.\ Government work not protected by U.S.\ copyright}
\\[2ex]
\noindent{\bf Copyright notice 2:}\\
For papers in which all authors are employed by a Crown government (UK, Canada, and Australia), the copyright notice is:\\
{978-1-7281-6662-9/20/\$31.00 {\copyright}2020 Crown}
\\[2ex]
\noindent{\bf Copyright notice 3:}\\
For papers in which all authors are employed by the European Union, the copyright notice is:\\
{978-1-7281-6662-9/20/\$31.00 {\copyright}2020 European Union}
\\[2ex]
\noindent{\bf Copyright notice 4:}\\
For all other papers the copyright notice is:\\
{978-1-7281-6662-9/20/\$31.00 {\copyright}2020 IEEE}

\section{Formatting your paper}
\label{sec:format}

All printed material, including text, illustrations, and charts, must be kept
within a print area of 7 inches (178 mm) wide by 9 inches (229 mm) high. Do
not write or print anything outside the print area. The top margin must be 1
inch (25 mm), except for the title page, and the left margin must be 0.75 inch
(19 mm).  All {\it text} must be in a two-column format. Columns are to be 3.39
inches (86 mm) wide, with a 0.24 inch (6 mm) space between them. Text must be
fully justified.

\section{PAGE TITLE SECTION}
\label{sec:pagestyle}

The paper title (on the first page) should begin 1.38 inches (35 mm) from the
top edge of the page, centered, completely capitalized, and in Times 14-point,
boldface type.  The authors' name(s) and affiliation(s) appear below the title
in capital and lower case letters. Note that double blind review is conducted and Authors Names and Affiliation only should appear in final paper if accepted. Papers with multiple authors and
affiliations may require two or more lines for this information.

\section{TYPE-STYLE AND FONTS}
\label{sec:typestyle}

To achieve the best rendering both in the proceedings and from the CD-ROM, we
strongly encourage you to use Times-Roman font.  In addition, this will give
the proceedings a more uniform look.  Use a font that is no smaller than nine
point type throughout the paper, including figure captions.

In nine point type font, capital letters are 2 mm high.  {\bf If you use the
smallest point size, there should be no more than 3.2 lines/cm (8 lines/inch)
vertically.}  This is a minimum spacing; 2.75 lines/cm (7 lines/inch) will make
the paper much more readable.  Larger type sizes require correspondingly larger
vertical spacing.  Please do not double-space your paper.  True-Type 1 fonts
are preferred.

The first paragraph in each section should not be indented, but all the
following paragraphs within the section should be indented as these paragraphs
demonstrate.

\section{MAJOR HEADINGS}
\label{sec:majhead}

Major headings, for example, "1. Introduction", should appear in all capital
letters, bold face if possible, centered in the column, with one blank line
before, and one blank line after. Use a period (".") after the heading number,
not a colon.

\subsection{Subheadings}
\label{ssec:subhead}

Subheadings should appear in lower case (initial word capitalized) in
boldface.  They should start at the left margin on a separate line.

\subsubsection{Sub-subheadings}
\label{sssec:subsubhead}

Sub-subheadings, as in this paragraph, are discouraged. However, if you
must use them, they should appear in lower case (initial word
capitalized) and start at the left margin on a separate line, with paragraph
text beginning on the following line.  They should be in italics.

\section{PRINTING YOUR PAPER}
\label{sec:print}

Print your properly formatted text on high-quality, 8.5 x 11-inch white printer
paper. A4 paper is also acceptable, but please leave the extra 0.5 inch (12 mm)
empty at the BOTTOM of the page and follow the top and left margins as
specified.  If the last page of your paper is only partially filled, arrange
the columns so that they are evenly balanced if possible, rather than having
one long column.

In LaTeX, to start a new column (but not a new page) and help balance the
last-page column lengths, you can use the command ``$\backslash$pagebreak'' as
demonstrated on this page (see the LaTeX source below).

\section{PAGE NUMBERING}
\label{sec:page}

Please do {\bf not} paginate your paper.  Page numbers, session numbers, and
conference identification will be inserted when the paper is included in the
proceedings.

\section{ILLUSTRATIONS, GRAPHS, AND PHOTOGRAPHS}
\label{sec:illust}

Illustrations must appear within the designated margins.  They may span the two
columns.  If possible, position illustrations at the top of columns, rather
than in the middle or at the bottom.  Caption and number every illustration.
All halftone illustrations must be clear black and white prints.  Colors may be
used, but they should be selected so as to be readable when printed on a
black-only printer.

Since there are many ways, often incompatible, of including images (e.g., with
experimental results) in a LaTeX document, below is an example of how to do
this \cite{Lamp86}.

% Below is an example of how to insert images. Delete the ``\vspace'' line,
% uncomment the preceding line ``\centerline...'' and replace ``imageX.ps''
% with a suitable PostScript file name.
% -------------------------------------------------------------------------
\begin{figure}[htb]

\begin{minipage}[b]{1.0\linewidth}
  \centering
  \centerline{\includegraphics[width=8.5cm]{image1}}
%  \vspace{2.0cm}
  \centerline{(a) Result 1}\medskip
\end{minipage}
%
\begin{minipage}[b]{.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image3}}
%  \vspace{1.5cm}
  \centerline{(b) Results 3}\medskip
\end{minipage}
\hfill
\begin{minipage}[b]{0.48\linewidth}
  \centering
  \centerline{\includegraphics[width=4.0cm]{image4}}
%  \vspace{1.5cm}
  \centerline{(c) Result 4}\medskip
\end{minipage}
%
\caption{Example of placing a figure with experimental results.}
\label{fig:res}
%
\end{figure}

% To start a new column (but not a new page) and help balance the last-page
% column length use \vfill\pagebreak.
% -------------------------------------------------------------------------
\vfill
\pagebreak


\section{FOOTNOTES}
\label{sec:foot}

Use footnotes sparingly (or not at all!) and place them at the bottom of the
column on the page on which they are referenced. Use Times 9-point type,
single-spaced. To help your readers, avoid using footnotes altogether and
include necessary peripheral observations in the text (within parentheses, if
you prefer, as in this sentence).


\section{COPYRIGHT FORMS}
\label{sec:copyright}

You must include your fully completed, signed IEEE copyright release form when
you submit your paper. We {\bf must} have this form before your paper can be
published in the proceedings.  The copyright form is available as a Word file,
a PDF file, and an HTML file. You can also use the form sent with your author
kit.
